Mesh Neural Networks for SE(3)-Equivariant Hemodynamics Estimation on the Artery Wall

Computational fluid dynamics (CFD) is a valuable asset for patient-specific cardiovascular-disease diagnosis and prognosis, but its high computational demands hamper its adoption in practice. Machine-learning methods that estimate blood flow in individual patients could accelerate or replace CFD simulation to overcome these limitations. In this work, we consider the estimation of vector-valued quantities on the wall of three-dimensional geometric artery models. We employ group equivariant graph convolution in an end-to-end SE(3)-equivariant neural network that operates directly on triangular surface meshes and makes efficient use of training data. We run experiments on a large dataset of synthetic coronary arteries and find that our method estimates directional wall shear stress (WSS) with an approximation error of 7.6% and normalised mean absolute error (NMAE) of 0.4% while up to two orders of magnitude faster than CFD. Furthermore, we show that our method is powerful enough to accurately predict transient, vector-valued WSS over the cardiac cycle while conditioned on a range of different inflow boundary conditions. These results demonstrate the potential of our proposed method as a plugin replacement for CFD in the personalised prediction of hemodynamic vector and scalar fields.

==> figures/bct.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{figures/bct.png}
    \caption{\textbf{Conditional, pulsatile} single-artery WSS prediction. GEM-GCN is conditioned on coronary blood flow and maps boundary conditions to according wall shear stress.}
    \label{fig:bct}
\end{figure}

==> figures/edge.tex <==
\begin{wrapfigure}[8]{r}{0.4\columnwidth}
    \includegraphics[width=0.4\columnwidth]{figures/edge.png}
    \caption{\textbf{Graph edge} construction from a mesh}
    \label{fig:edge}
\end{wrapfigure}

==> figures/pressure.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/pressure.png}
    \caption{\textbf{Influence of receptive field.} We train three GEM-GCN architectures with two, one, a no pooling layers on ground-truth pressure for two samples of the steady-flow single-artery dataset. For the sample in the left column, the theoretical receptive field is visualised.}
    \label{fig:pressure}
\end{figure}

==> figures/showcase.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/showcase.png}  % PDF not possible with fade effects
    \caption{\textbf{Pulsatile} WSS predictions for a single artery. GEM-GCN returns a vector field for each discrete point in time over one cardiac cycle.}
    \label{fig:showcase}
\end{figure*}

==> plots/bct.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{plots/bct.png}
    \caption{\textbf{Conditional, pulsatile} single (top) and bifurcating (bottom) artery WSS prediction error across the test split over time. Five boundary conditions per artery are contained as separate data points. Maximum WSS magnitude is indicated in yellow.}
    \label{plt:bct}
\end{figure}

==> tables/wallclock.tex <==
\begin{table}[h]
	\begin{center}
    	\caption{\textbf{Training time until convergence} measured in number of epochs and wall-clock time of parallelised training on two NVIDIA A40 GPUs.}
    	\renewcommand{\arraystretch}{1.3}
    	\begin{tabular}{@{}cccccc@{}}
    		\toprule
    		& \multicolumn{2}{c}{\# epochs} && \multicolumn{2}{c}{Wall-clock time [h]}\\
    		\cmidrule{2-3} \cmidrule{5-6}
    		& single & bifurcating && single & bifurcating\\
    		\midrule
    		IsoGCN & 1145 & \phantom{0}270 && 10:03 & \phantom{0}6:13\\
    		AttGCN & 1470 & \phantom{0}660 && 31:18 & 30:48\\
    		PointNet\texttt{++} & 3920 & 1600 && 20:48 & 35:01\\
    		\midrule
    		GEM-GCN & \phantom{0}700 & \phantom{0}165 && 22:24 & 15:57\\
    		PointNet\texttt{++}$^\ddagger$ & 6735 & 3330 && 31:29 & 57:16\\
    		\bottomrule
    		\multicolumn{6}{l}{$^\ddagger$ trained under data augmentation (random rotation in 3D)}
    	\end{tabular}
    	\label{tab:wallclock}
	\end{center}
\end{table}
